On the Expressivity of Typed Concurrent Calculi

This thesis embarks on a comprehensive exploration of formal computational models that underlie typed programming languages. We focus on programming calculi, both functional (sequential) and concurrent, as they provide a compelling rigorous framework for evaluating program semantics and for developing analyses and program verification techniques. This is the full version of the thesis containing appendices.

==> 0-misc/dedication.tex <==
%\vspace*{-0.4cm}
%\vspace*{4cm}
\dedication{\epigraph{ADD A QUOTE}{MOST LIKELY DOUGLAS ADAMS}}

%\begin*{dedication}
%I have something to say.
%\end*{dedication}








==> 0-misc/glossary.tex <==
\chapter*{Glossary}\markboth{Glossary}{Glossary}
\addcontentsline{toc}{chapter}{Glossary}

%\renewcommand{\imagepath}[1]{\fname{0-misc/images/#1}}
\graphicspath{{./0-misc/images/}}


\section*{Conventions}
The following conventions are used in this thesis for notation
and symbols:
\begin{itemize}
\item A lower case character typeset in boldface, e.g., $\mathbf{x}$,
   represents a column vector.
\item The number of elements in a vector $\mathbf{x}$ is indicated by
   $n_{\mathbf{x}}$.
\item \ldots
\end{itemize}

\section*{List of symbols and notations}
Below follows a list of the most frequently used symbols and notations
in this thesis. Symbols particular to power network applications
are explained only in the relevant chapters.

\vspace*{-0.4cm}\begin{tabbing}
\hspace*{3.5cm}\=\kill\\
$ \mathbf{A}  $ \> system matrices of linear time-invariant models \\
\\[-0.1cm]
$ \mathbf{B}  $ \> input matrices of linear time-invariant models \\
\\[-0.1cm]
$ \mathbf{E}_1 $ \> matrices of mixed-logical dynamic models \\
\end{tabbing}

\vspace*{-0.7cm}
\section*{List of abbreviations}
The following abbreviations are used in this thesis:
\begin{tabbing}
\hspace*{4cm}\=\kill
AVR \> Automatic Voltage Regulator\\
DAE \> Differential-Algebraic Equations\\
FACTS \> Flexible Alternating-Current Transmission System\\
MPC \> Model Predictive Control\\
\ldots \> \ldots
\end{tabbing}


==> 0-misc/preface.tex <==
\clearemptydoublepage

\chapter*{Acknowledgement}
% to make sure that TOC fits on 3 pages:
\addtocontents{toc}{\vspace*{-0.9cm}}
\addcontentsline{toc}{chapter}{Preface}

%\renewcommand{\imagepath}[1]{\fname{0-misc/images/#1}}
\graphicspath{{./0-misc/images/}}

\vspace*{-0.4cm}


Acknowledgement

==> 1-intro/chapters/chaps.tex <==


\chapter{Non-Deterministic Functions as   Non-Deterministic Processes}\label{ch2}




\chapter{Types and Terms Translated:  Unrestricted Resources in Encoding  Functions as Processes}\label{ch3}



\chapter{Typed Non-determinism in Functional and Concurrent Calculi}\label{ch4}



\chapter{Termination in Concurrency, Revisited}\label{ch5}




==> 2-LMCS/figure.tex <==
 \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Circle [id:dp7964522619162369] 
\draw   (22,105.25) .. controls (22,85.78) and (37.78,70) .. (57.25,70) .. controls (76.72,70) and (92.5,85.78) .. (92.5,105.25) .. controls (92.5,124.72) and (76.72,140.5) .. (57.25,140.5) .. controls (37.78,140.5) and (22,124.72) .. (22,105.25) -- cycle ;
%Shape: Circle [id:dp2429873823346096] 
\draw   (186.5,105.5) .. controls (186.5,86.17) and (202.17,70.5) .. (221.5,70.5) .. controls (240.83,70.5) and (256.5,86.17) .. (256.5,105.5) .. controls (256.5,124.83) and (240.83,140.5) .. (221.5,140.5) .. controls (202.17,140.5) and (186.5,124.83) .. (186.5,105.5) -- cycle ;
%Shape: Circle [id:dp9380332011019401] 
\draw   (104,223) .. controls (104,200.36) and (122.36,182) .. (145,182) .. controls (167.64,182) and (186,200.36) .. (186,223) .. controls (186,245.64) and (167.64,264) .. (145,264) .. controls (122.36,264) and (104,245.64) .. (104,223) -- cycle ;
%Shape: Circle [id:dp34779892344880925] 
\draw   (132,212) .. controls (132,200.95) and (140.95,192) .. (152,192) .. controls (163.05,192) and (172,200.95) .. (172,212) .. controls (172,223.05) and (163.05,232) .. (152,232) .. controls (140.95,232) and (132,223.05) .. (132,212) -- cycle ;
%Straight Lines [id:da4684388085916382] 
\draw    (79,105) -- (199.5,106.48) ;
\draw [shift={(201.5,106.5)}, rotate = 180.7] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da836225068889987] 
\draw    (211.5,127) -- (156.64,206.35) ;
\draw [shift={(155.5,208)}, rotate = 304.65999999999997] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da16098165722112578] 
\draw    (74.5,126.5) -- (148.14,206.03) ;
\draw [shift={(149.5,207.5)}, rotate = 227.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (48.5,96.4) node [anchor=north west][inner sep=0.75pt]    {$\lamrfail$};
% Text Node
\draw (215,97.4) node [anchor=north west][inner sep=0.75pt]    {$\lamrsharfail$};
% Text Node
\draw (117,224.9) node [anchor=north west][inner sep=0.75pt]    {$\spi$};
% Text Node
\draw (121,17.9) node [anchor=north west][inner sep=0.75pt]    {$
                                                                    \begin{aligned}
                                                                        \text{Thm }  \ref{ch2thm:preservencintolamrfail2}\\
                                                                        \text{Thm } \ref{ch2l:app_completenessone}\\
                                                                        \text{Thm } \ref{ch2l:soundnessone}\\
                                                                        \text{Thm } \ref{ch2proof:app_successsensce}\\
                                                                    \end{aligned}$};
% Text Node
\draw (203,152.9) node [anchor=north west][inner sep=0.75pt]    {$
                                                                    \begin{aligned}
                                                                        \text{Thm }  \ref{ch2t:preservationtwo}\\
                                                                        \text{Thm } \ref{ch2l:app_completenesstwo}\\
                                                                        \text{Thm } \ref{ch2l:app_soundnesstwo}\\
                                                                        \text{Thm } \ref{ch2proof:successsenscetwo}\\
                                                                    \end{aligned}$};


\end{tikzpicture}
